Delay-Optimal Forwarding and Computation Offloading for Service Chain Tasks

Emerging edge computing paradigms enable heterogeneous devices to collaborate on complex computation applications. However, for congestible links and computing units, delay-optimal forwarding and offloading for service chain tasks (e.g., DNN with vertical split) in edge computing networks remains an open problem. In this paper, we formulate the service chain forwarding and offloading problem with arbitrary topology and heterogeneous transmission/computation capability, and aim to minimize the aggregated network cost. We consider congestion-aware nonlinear cost functions that cover various performance metrics and constraints, such as average queueing delay with limited processor capacity. We solve the non-convex optimization problem globally by analyzing the KKT condition and proposing a sufficient condition for optimality. We then propose a distributed algorithm that converges to the global optimum. The algorithm adapts to changes in input rates and network topology, and can be implemented as an online algorithm. Numerical evaluation shows that our method significantly outperforms baselines in multiple network instances, especially in congested scenarios.

==> ACM_files/macros_acm.tex <==
%\usepackage{amsmath, amssymb}
%\usepackage{mathtools}
%\usepackage{caption}
%\usepackage{amsthm,multirow,color,amsfonts}
%\usepackage{tabulary}
%\usepackage{subfigure}
%\usepackage{graphicx}
%\usepackage{setspace}
%\usepackage{enumerate}
\usepackage{comment}
%\usepackage{cite}
%\usepackage{bm}
%\usepackage{bbm}
%\usepackage[linesnumbered]{algorithm2e}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
%\usepackage[noend]{algpseudocode} % I think we should have ends for algorithms
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother
	

\DeclareMathOperator*{\Phit}{P_{\sf Hit}}
\DeclareMathOperator*{\Pmiss}{P_{\sf Miss}}


\def\rt{\theta}
\def\ro{\omega}
\def\rO{\Omega}


\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\norm}[1]{\| #1 \|}                 
\newtheorem{theo}{Theorem}
\newtheorem{defi}{Definition}
\newtheorem{assu}{Assumption}
\newtheorem{prop}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{note}{Note}
\newtheorem{cor}{Corollary}
\newtheorem{ques}{Questions}
\newtheorem{lem}{Lemma}
\newtheorem{exam}{Example}

\newcommand{\chr}[1]{{\em \color{red} #1}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\RHS}{\sf RHS}
\DeclareMathOperator*{\LHS}{\sf LHS}

%\DeclareMathOperator*{\sinr}{{\sf{SINR}}}    
\DeclareMathOperator*{\SINR}{{\mathrm{SINR}}}  
\DeclareMathOperator*{\sir}{\sf{SIR}}    
\DeclareMathOperator*{\SIR}{\mathrm{SIR}}
\DeclareMathOperator*{\snr}{\sf{SNR}}  
\DeclareMathOperator*{\SNR}{\mathrm{SNR}}   

\DeclareMathOperator*{\SR}{\sf{SR}} %source routing
\DeclareMathOperator*{\HH}{\sf{HH}} %hop by hop routing
\DeclareMathOperator*{\LP}{\sf{LP}} %linear program

\DeclareMathOperator*{\Find}{F_{\sf{indep.}}}
\DeclareMathOperator*{\Fneg}{F_{\sf{neg-dep.}}}


\DeclareMathOperator*{\Shannon}{\sf{Shannon}}
\DeclareMathOperator*{\MQAM}{\sf{MQAM}}

%\DeclareMathOperator*{\Dpwl}{\mathcal{D}_{\text piecewise-linear}}
\DeclareMathOperator*{\Dpwl}{\mathcal{D}_{\text pwl}}


\DeclareMathOperator*{\DD}{\sf{D2D}}  
\DeclareMathOperator*{\BS}{\sf{BS}}    
\DeclareMathOperator*{\PPP}{\sf{PPP}} 

\DeclareMathOperator\erf{erf}
\DeclareMathOperator*{\Q}{\rm Q}

\DeclareMathOperator*{\CSMA}{\sf CSMA}
\DeclareMathOperator*{\Poisson}{\sf Poisson}
\newcommand{\poisscdf}{{\sf{poisscdf}}}
\newcommand{\normcdf}{{\sf{normcdf}}}
\newcommand{\poisspmf}{{\sf{poisspmf}}}
\newcommand{\poissinv}{{\sf{poissinv}}}

\DeclareMathOperator*{\Rdd}{R_{\sf{D2D}}} 
\DeclareMathOperator*{\Rdds}{R_{\sf{D2D}}^2} 

\DeclareMathOperator*{\mhc}{\sf MHC}
\DeclareMathOperator*{\tx}{$\lambda_T$}%density of active transmitters
\DeclareMathOperator*{\rx}{$\lambda_R$}

\DeclareMathOperator*{\PGFL}{\sf{PGFL}} 
\DeclareMathOperator*{\CCDF}{\sf{CCDF}} 

\newcommand{\Num}{{\rm Num}}
\newcommand{\Den}{{\rm Den}}

%%usefull commands%%%%%%%%%%%
\newcommand{\parenv}[1]{\left( {#1} \right)}
\newcommand{\floorenv}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\ceilenv}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\mathset}[1]{\left\{ {#1} \right\}}
\newcommand{\sparenv}[1]{\left[ {#1} \right]}
\newcommand{\Ex}[1]{\mathbb{E}\!\left[{#1} \right]}
\newcommand{\Exv}[1]{\mathbb{E}_{\nu}\!\left[{#1} \right]}
\newcommand{\Var}[1]{\mathrm{Var}\!\left[{#1} \right]}
\newcommand{\td}{\tilde{d}}
\newcommand{\eqdef}{\triangleq}



\newcommand{\z}{z_{p_{k+1} p_k, p_l}(i,p)}        
\newcommand{\tp}{t_{p_{k+1} p_k}(i,p)}                            

\newcommand{\zz}{z_{p_{k+1} p_k}(i,p)} 
\newcommand{\zzopt}{z_{p_{k+1} p_k}^{*}(i,p)}   
\newcommand{\zzoptrelaxed}{z_{p_{k+1} p_k}^{**}(i,p)} 
\newcommand{\Dopt}{D^{*}}
\newcommand{\Doptrelaxed}{D^{**}}



\newcommand{\MD}{{\rm CITADEL} }%maybe the algorithm



\newcommand{\derya}[1]{\textit{\textcolor{blue}{Derya: #1}}}
\newcommand{\volkan}[1]{\textit{\textcolor{red}{Volkan: #1}}}
\newcommand{\jinkun}[1]{\textit{\textcolor{blue}{Jinkun: #1}}}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
